Curriculum: A Broad-Coverage Benchmark for Linguistic Phenomena in Natural Language Understanding

In the age of large transformer language models, linguistic evaluation play an important role in diagnosing models' abilities and limitations on natural language understanding. However, current evaluation methods show some significant shortcomings. In particular, they do not provide insight into how well a language model captures distinct linguistic skills essential for language understanding and reasoning. Thus they fail to effectively map out the aspects of language understanding that remain challenging to existing models, which makes it hard to discover potential limitations in models and datasets. In this paper, we introduce Curriculum as a new format of NLI benchmark for evaluation of broad-coverage linguistic phenomena. Curriculum contains a collection of datasets that covers 36 types of major linguistic phenomena and an evaluation procedure for diagnosing how well a language model captures reasoning skills for distinct types of linguistic phenomena. We show that this linguistic-phenomena-driven benchmark can serve as an effective tool for diagnosing model behavior and verifying model learning quality. In addition, our experiments provide insight into the limitation of existing benchmark datasets and state-of-the-art models that may encourage future research on re-designing datasets, model architectures, and learning objectives.

==> tables/ontology_table.tex <==
% \begin{table*}[]
% \centering
% \scalebox{0.75}{

\section{Selected Tasks in NLP Few-shot Gym}
\label{sec:all_tasks_table}
\scriptsize


\begin{longtable}{lllll}
\caption{Tasks in NLP Few-shot Gym.}\label{tab:ontology}\\
\toprule
\textbf{Task Name} & \textbf{Ontology} & \textbf{Reference} \\
\midrule
\endfirsthead
\toprule
\textbf{Task Name} & \textbf{Ontology} & \textbf{Reference} \\
\midrule
\endhead
\bottomrule \multicolumn{4}{r}{Continued on next page} \\
\endfoot
% \bottomrule
% \vspace{1cm}
\endlastfoot
acronym\_identification &	other &	\citealt{pouran-ben-veyseh-etal-2020-acronym}	\\
ade\_corpus\_v2-classification &	cls/other &	\citealt{GURULINGAPPA2012885}	\\
ade\_corpus\_v2-dosage &	other/slot filling & \citealt{GURULINGAPPA2012885}	\\
ade\_corpus\_v2-effect &	other/slot filling & \citealt{GURULINGAPPA2012885}	\\
adversarialqa &	qa/machine reading comprehension &	\citealt{bartolo-etal-2020-beat}	\\
aeslc &	cg/summarization & \citealt{zhang-tetreault-2019-email}	\\
ag\_news &	cls/topic &	\href{http://groups.di.unipi.it/~gulli/AG_corpus_of_news_articles.html}{Gulli (link)}	\\
ai2\_arc &	qa/multiple-choice qa &	\citealt{Clark2018ThinkYH}	\\
amazon\_polarity &	cls/sentiment analysis & \citealt{McAuley2013HiddenFA}	\\
anli &	cls/nli & \citealt{nie-etal-2020-adversarial}	\\
app\_reviews &	other/regression &	Missing\\ %\citealt{app-review}	\\
aqua\_rat &	qa/multiple-choice qa &	\citealt{ling-etal-2017-program}	\\
art (abductive nli) &	other &	\citealt{bhagavatula2020abductive}	\\
aslg\_pc12 &	other &	\citealt{Othman2012EnglishASLGP}	\\
biomrc &	qa/machine reading comprehension &	\citealt{pappas-etal-2020-biomrc}	\\
blimp-anaphor\_gender\_agreement &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-anaphor\_number\_agreement &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-determiner\_noun\_agreement\_with\_adj\_irregular\_1 &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-ellipsis\_n\_bar\_1 &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-ellipsis\_n\_bar\_2 &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-existential\_there\_quantifiers\_1 &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-irregular\_past\_participle\_adjectives &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-sentential\_negation\_npi\_licensor\_present &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-sentential\_negation\_npi\_scope &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
blimp-wh\_questions\_object\_gap &	other/linguistic phenomenon & \citealt{warstadt2019blimp}	\\
boolq &	qa/binary &	\citealt{clark-etal-2019-boolq}	\\
break-QDMR &	other &	\citealt{wolfson-etal-2020-break}	\\
break-QDMR-high-level &	other & \citealt{wolfson-etal-2020-break}	\\
circa &	cls/other &	\citealt{louis-etal-2020-id}	\\
climate\_fever &	cls/fact checking &	\citealt{Diggelmann2020CLIMATEFEVERAD}	\\
codah &	qa/multiple-choice qa &	\citealt{chen-etal-2019-codah}	\\
common\_gen &	other &	\citealt{lin-etal-2020-commongen}	\\
commonsense\_qa &	qa/multiple-choice qa &	\citealt{talmor-etal-2019-commonsenseqa}	\\
cos\_e &	other/generate explanation & \citealt{rajani-etal-2019-explain}	\\
cosmos\_qa &	qa/multiple-choice qa &	\citealt{huang-etal-2019-cosmos}	\\
crawl\_domain &	other &	\citealt{zhang-etal-2020-semi}	\\
crows\_pairs &	other &	\citealt{nangia-etal-2020-crows}	\\
dbpedia\_14 &	cls/topic &	\citealt{Lehmann2015DBpediaA}	\\
definite\_pronoun\_resolution &	other &	\citealt{rahman-ng-2012-resolving}	\\
discovery &	cls/other &	\citealt{sileo-etal-2019-mining}	\\
dream &	qa/multiple-choice qa &	\citealt{sun-etal-2019-dream}	\\
duorc &	qa/machine reading comprehension &	\citealt{saha-etal-2018-duorc}	\\
e2e\_nlg\_cleaned &	other &	\citealt{dusek.etal2020:csl, dusek-etal-2019-semantic}	\\
eli5-askh &	qa/long-form qa & \citealt{fan-etal-2019-eli5}	\\
eli5-asks &	qa/long-form qa & \citealt{fan-etal-2019-eli5}	\\
eli5-eli5 &	qa/long-form qa & \citealt{fan-etal-2019-eli5}	\\
emo &	cls/emotion & \citealt{chatterjee-etal-2019-semeval}	\\
emotion &	cls/emotion & \citealt{saravia-etal-2018-carer}	\\
empathetic\_dialogues &	cg/dialogue & \citealt{rashkin-etal-2019-towards}	\\
ethos-directed\_vs\_generalized &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-disability &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-gender &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-national\_origin &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-race &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-religion &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
ethos-sexual\_orientation &	cls/hate speech detection &	\citealt{Mollas2020ETHOSAO}	\\
financial\_phrasebank &	cls/sentiment analysis &	\citealt{financial-phrasebank}	\\
freebase\_qa &	qa/closed-book qa &	\citealt{jiang-etal-2019-freebaseqa}	\\
gigaword &	cg/summarization &	\citealt{napoles-etal-2012-annotated}	\\
glue-cola &	cls/other &	\citealt{warstadt-etal-2019-neural}	\\
glue-mnli &	cls/nli & \citealt{williams-etal-2018-broad}	\\
glue-mrpc &	cls/paraphrase & \citealt{dolan-brockett-2005-automatically}\\
glue-qnli &	cls/nli &	\citealt{rajpurkar-etal-2016-squad}	\\
glue-qqp &	cls/paraphrase & \href{http://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}	\\
glue-rte &	cls/nli &	\begin{tabular}[c]{@{}l@{}}\citealt{dagan2005pascal, bar2006second}\\\citealt{giampiccolo2007third, bentivogli2009fifth}\end{tabular}	\\
glue-sst2 &	cls/sentiment analysis &	\citealt{socher-etal-2013-recursive}	\\
glue-wnli &	cls/nli & \citealt{levesque2012winograd}	\\
google\_wellformed\_query &	cls/other &	\citealt{faruqui-das-2018-identifying}	\\
hate\_speech18 &	cls/hate speech detection &	\citealt{gibert2018hate}	\\
hate\_speech\_offensive &	cls/hate speech detection &	\citealt{hateoffensive}	\\
hatexplain &	cls/hate speech detection &	\citealt{mathew2020hatexplain}	\\
health\_fact &	cls/fact checking &	\citealt{kotonya-toni-2020-explainable-automated}	\\
hellaswag &	qa/multiple-choice qa &	\citealt{zellers-etal-2019-hellaswag}	\\
hotpot\_qa &	qa/machine reading comprehension &	\citealt{yang-etal-2018-hotpotqa}	\\
imdb &	cls/sentiment analysis & \citealt{maas-etal-2011-learning}	\\
jeopardy &	qa/closed-book qa &	\href{https://www.reddit.com/r/datasets/comments/1uyd0t/200000_jeopardy_questions_in_a_json_file/}{(link)}	\\
kilt\_ay2 &	other/entity linking &	\citealt{hoffart-etal-2011-robust}	\\
kilt\_fever &	cls/fact checking &	\citealt{thorne-etal-2018-fever}	\\
kilt\_hotpotqa &	qa/closed-book qa &	\citealt{yang-etal-2018-hotpotqa}	\\
kilt\_nq &	qa/closed-book qa &	\citealt{kwiatkowski-etal-2019-natural}	\\
kilt\_trex &	qa/closed-book qa &	\citealt{elsahar-etal-2018-rex}	\\
kilt\_wow &	cg/dialogue &	\citealt{dinan2018wizard}	\\
kilt\_zsre &	qa/closed-book qa &	\citealt{levy-etal-2017-zero}	\\
lama-conceptnet &	qa/closed-book qa &	\citealt{petroni-etal-2019-language,petroni2020how}	\\
lama-google\_re &	qa/closed-book qa &	\citealt{petroni-etal-2019-language,petroni2020how}	\\
lama-squad &	qa/closed-book qa &	\citealt{petroni-etal-2019-language,petroni2020how}	\\
lama-trex &	qa/closed-book qa &	\citealt{petroni-etal-2019-language,petroni2020how}	\\
liar &	cls/fact checking &	\citealt{wang-2017-liar}	\\
limit &	other &	\citealt{manotas-etal-2020-limit}	\\
math\_qa &	qa/multiple-choice qa &	\citealt{amini-etal-2019-mathqa}	\\
mc\_taco &	qa/binary &	\citealt{zhou-etal-2019-going}	\\
medical\_questions\_pairs &	cls/paraphrase & \citealt{medical-qqp}	\\
mocha &	other/regression &	\citealt{chen-etal-2020-mocha}	\\
multi\_news &	cg/summarization & \citealt{fabbri-etal-2019-multi}	\\
numer\_sense &	qa/closed-book qa &	\citealt{lin-etal-2020-birds}	\\
onestop\_english &	cls/other &	\citealt{vajjala-lucic-2018-onestopenglish}	\\
openbookqa &	qa/multiple-choice qa &	\citealt{mihaylov-etal-2018-suit}	\\
paws &	cls/paraphrase & \citealt{zhang-etal-2019-paws}	\\
piqa &	other &	\citealt{Bisk2020}	\\
poem\_sentiment &	cls/sentiment analysis & \citealt{sheng-uthus-2020-investigating}	\\
proto\_qa &	other &	\citealt{boratko-etal-2020-protoqa}	\\
qa\_srl &	other &	\citealt{he-etal-2015-question}	\\
qasc &	qa/multiple-choice qa &	\citealt{Khot_Clark_Guerquin_Jansen_Sabharwal_2020}	\\
quail &	qa/multiple-choice qa &	\citealt{Rogers_Kovaleva_Downey_Rumshisky_2020}	\\
quarel &	qa/multiple-choice qa &	\citealt{Tafjord_Clark_Gardner_Yih_Sabharwal_2019}	\\
quartz-no\_knowledge &	qa/multiple-choice qa &	\citealt{tafjord-etal-2019-quartz}	\\
quartz-with\_knowledge &	qa/multiple-choice qa &	\citealt{tafjord-etal-2019-quartz}	\\
quoref &	qa/machine reading comprehension &	\citealt{dasigi-etal-2019-quoref}	\\
race-high &	qa/multiple-choice qa &	\citealt{lai-etal-2017-race}	\\
race-middle &	qa/multiple-choice qa &	\citealt{lai-etal-2017-race}	\\
reddit\_tifu-title &	cg/summarization &	\citealt{kim-etal-2019-abstractive}	\\
reddit\_tifu-tldr &	cg/summarization &	\citealt{kim-etal-2019-abstractive}	\\
ropes &	qa/machine reading comprehension &	\citealt{lin-etal-2019-reasoning}	\\
rotten\_tomatoes &	cls/sentiment analysis & \citealt{pang-lee-2005-seeing}	\\
samsum &	cg/summarization &	\citealt{gliwa-etal-2019-samsum}	\\
scicite &	cls/other &	\citealt{cohan-etal-2019-structural}	\\
sciq &	qa/multiple-choice qa &	\citealt{welbl-etal-2017-crowdsourcing}	\\
scitail &	cls/nli & \citealt{scitail}	\\
search\_qa &	qa/closed-book qa &	\citealt{Dunn2017SearchQAAN}	\\
sick &	cls/nli &	\citealt{marelli-etal-2014-sick}	\\
sms\_spam &	cls/other &	\citealt{sms_spam}	\\
social\_i\_qa &	qa/multiple-choice qa &	\citealt{sap-etal-2019-social}	\\
spider &	cg/other &	\citealt{yu-etal-2018-spider}	\\
squad-no\_context &	qa/closed-book qa &	\citealt{rajpurkar-etal-2016-squad}	\\
squad-with\_context &	qa/machine reading comprehension &	\citealt{rajpurkar-etal-2016-squad}	\\
superglue-cb &	cls/nli & \citealt{Marneffe_Simons_Tonhauser_2019}	\\
superglue-copa &	qa/multiple-choice qa &	\citealt{gordon-etal-2012-semeval} \\
superglue-multirc &	qa/multiple-choice qa &	\citealt{khashabi-etal-2018-looking}	\\
superglue-record &	qa/machine reading comprehension & \citealt{Zhang2018ReCoRDBT}	\\
superglue-rte &	cls/nli & \begin{tabular}[c]{@{}l@{}}\citealt{dagan2005pascal, bar2006second}\\\citealt{giampiccolo2007third, bentivogli2009fifth}\end{tabular}	\\
superglue-wic &	cls/other &	\citealt{pilehvar-camacho-collados-2019-wic}	\\
superglue-wsc &	cls/other &	\citealt{levesque2012winograd}	\\
swag &	qa/multiple-choice qa &	\citealt{zellers-etal-2018-swag}	\\
tab\_fact &	cls/fact checking &	\citealt{Chen2020TabFact}	\\
trec &	cls/other &	\citealt{li-roth-2002-learning,hovy-etal-2001-toward}	\\
trec-finegrained &	cls/other &	\citealt{li-roth-2002-learning,hovy-etal-2001-toward}	\\
tweet\_eval-emoji &	cls/emotion & \citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-emotion &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-hate &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-irony &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-offensive &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-sentiment &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-stance\_abortion &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-stance\_atheism &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-stance\_climate &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-stance\_feminist &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_eval-stance\_hillary &	cls/emotion &	\citealt{barbieri-etal-2020-tweeteval}	\\
tweet\_qa &	qa/machine reading comprehension &	\citealt{xiong-etal-2019-tweetqa}	\\
web\_questions &	qa/closed-book qa &	\citealt{berant-etal-2013-semantic}	\\
wiki\_auto &	cls/other &	\citealt{jiang-etal-2020-neural}	\\
wiki\_bio &	cg/other &	\citealt{lebret-etal-2016-neural}	\\
wiki\_qa &	cls/other &	\citealt{yang-etal-2015-wikiqa}	\\
wiki\_split &	cg/other & \citealt{botha-etal-2018-learning}	\\
wikisql &	cg/other &	\citealt{zhongSeq2SQL2017}	\\
wino\_grande &	qa/multiple-choice qa &	\citealt{Sakaguchi_Le_Bras_Bhagavatula_Choi_2020}	\\
wiqa &	qa/multiple-choice qa &	\citealt{tandon-etal-2019-wiqa}	\\
xsum &	cg/summarization &	\citealt{narayan-etal-2018-dont}	\\
yahoo\_answers\_topics &	cls/topic &	\href{https://webscope.sandbox.yahoo.com/catalog.php?datatype=l}{(link)}	\\
yelp\_polarity &	cls/sentiment analysis & \citealt{zhang2015character}; \href{https://www.yelp.com/dataset}{(link)}	\\
yelp\_review\_full &	other/regression &	\citealt{zhang2015character}; \href{https://www.yelp.com/dataset}{(link)}	\\
\bottomrule
\end{longtable}
\normalsize

% }
% \caption{Tasks in NLP Few-shot Gym.}
% \label{tab:ontology}
% \end{table*}

==> tables/q2.tex <==
\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{cccc}
\toprule
\textbf{Strategy} &  A1$_{acc}$ & A2$_{acc}$ & A3$_{acc}$  \\
\midrule
\multirow{1}{*}{None}       &   &   &   \\
\midrule
\multirow{1}{*}{Machine}    &   & 67.9($\Delta$) &  \\
\midrule
\multirow{1}{*}{Machine+}   &   &   &   \\
\midrule
\multirow{1}{*}{Human}      &  & 69.5($\Delta$)  &  \\
\midrule
\multirow{1}{*}{Human+}     &  &   &      \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of test task performance when different $\mathcal{T}_{train}$ sets are used in upstream learning. See text in Q2 for in-depth analysis.}
\label{tab:scaffold}
\end{table}

==> tables/splits.tex <==
\begin{table*}[]
\centering
\scalebox{0.65}{
\begin{tabular}{r|c||ccc|cccc|c}
\toprule
No. & Shorthand & $\mathcal{T}_{train}$ & $\mathcal{T}_{dev}$ & $\mathcal{T}_{test}$ & ARG(Multi) & ARG(MAML) & ARG(FoMAML) & ARG(Rept.) & Details \\\midrule
1    &   Random        &  120  &  20  &  20  &  $35.06\%$  & $28.50\%$  & $22.69\%$ & $25.90\%$ &    Fig.~\ref{fig:all}(a)  \\\midrule
2.1    & 45cls          &  45 cls.   &     {10 cls.}   &   {10 cls.}  &  $11.68\%$   &  $9.37\%$  & $10.28\%$ & $13.36\%$ & \multirow{3}{*}{Fig.~\ref{fig:classification-merge-test}}        \\
2.2    & 23cls+22non-cls          &  23 cls. + 22 non-cls.   &   {10 cls.}   &   {10 cls.}          &  $11.82\%$ & $9.69\%$ & $13.75\%$ & $14.34\%$&    \\
2.3    & 45non-cls         &  45 non-cls.   &    {10 cls.}   &   {10 cls.}     & $11.91\%$   & $9.33\%$ & $11.20\%$ & 
$14.14\%$&              \\\midrule
3.1    & Held-out-NLI  &   57 non-NLI cls.  &   /     &  8 NLI   &   $16.94\%$  & $12.30\%$ & $12.33\%$ & $14.46\%$ &  Fig.~\ref{fig:all}(b)\\
3.2    & Held-out-Para  &   61 non-Paraphrase cls.  &   /     &  4 Para. Iden.   &    $18.21\%$ & $17.90\%$ & $21.57\%$ & $19.72\%$ & Fig.~\ref{fig:all}(c) \\\midrule
4.1 & Held-out-MRC & 42 non-MRC QA & / & 9 MRC &$32.81\%$ & $27.28\%$ & $28.85\%$ & $28.85\%$ & Fig.~\ref{fig:all}(d) \\
4.2 & Held-out-MCQA & 29 non-MC QA & / & 22 MC QA & $12.20\%$ & $4.69\%$ &$6.73\%$ & $7.67\%$ & Fig.~\ref{fig:all}(e)\\\bottomrule
\end{tabular}
}
\caption{$(\mathcal{T}_{train}$,$\mathcal{T}_{dev}$,$\mathcal{T}_{test})$ partitions used in the study (full lists in Appendix~\ref{app:partitions}), and their ARG scores when upstream learning methods are applied. 
% Full lists of the tasks in the partitions are listed in Appendix~\ref{app:partitions}.
``cls.'' stands for ``classification'', ``Para. Iden.'' for ``paraphrase identification'', ``MRC'' for ``machine reading comprehension'' and ``MCQA'' for ``multiple-choice QA''.
}
\label{tab:splits}
\end{table*}

% \xiang{1) add column for direct fine-tune's absolute performance; 2) add a line to point to specific place in appendix for the details of the task partitions.}

% \\
% $^*$ ``cls.'' stands for ``classification'', ``Para. Iden.'' stands for ``paraphrase identification'', ``MRC'' for ``machine reading comprehension'' and ``MCQA'' for ``multiple-choice QA''.

==> tables/task_partitions.tex <==
% \clearpage

\section{Details about Task Partition}

\label{app:partitions}
\subsection{Partition 1. Random}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ['glue-mrpc', 'math_qa', 'quarel', 'e2e_nlg_cleaned', 'tweet_eval-stance_atheism', 'lama-squad', 'tab_fact', 'aqua_rat', 'tweet_eval-emoji', 'glue-wnli', 'codah', 'tweet_eval-offensive', 'wiki_qa', 'blimp-ellipsis_n_bar_1', 'openbookqa', 'sms_spam', 'acronym_identification', 'blimp-determiner_noun_agreement_with_adj_irregular_1', 'ethos-national_origin', 'spider', 'definite_pronoun_resolution', 'hellaswag', 'superglue-wsc', 'numer_sense', 'ade_corpus_v2-dosage', 'blimp-ellipsis_n_bar_2', 'kilt_ay2', 'squad-no_context', 'google_wellformed_query', 'xsum', 'wiqa', 'tweet_eval-stance_abortion', 'reddit_tifu-tldr', 'ade_corpus_v2-effect', 'qa_srl', 'ethos-religion', 'commonsense_qa', 'jeopardy', 'biomrc', 'superglue-multirc', 'ethos-race', 'eli5-askh', 'glue-qqp', 'paws', 'ethos-directed_vs_generalized', 'glue-sst2', 'mocha', 'tweet_eval-hate', 'glue-rte', 'blimp-anaphor_number_agreement', 'lama-conceptnet', 'hate_speech_offensive', 'superglue-wic', 'boolq', 'kilt_hotpotqa', 'quartz-no_knowledge', 'aslg_pc12', 'sick', 'tweet_eval-stance_climate', 'tweet_eval-sentiment', 'crows_pairs', 'glue-mnli', 'medical_questions_pairs', 'break-QDMR-high-level', 'qasc', 'imdb', 'ethos-gender', 'trec-finegrained', 'adversarialqa', 'onestop_english', 'web_questions', 'duorc', 'yelp_review_full', 'swag', 'proto_qa', 'scitail', 'tweet_eval-stance_feminist', 'limit', 'common_gen', 'scicite', 'blimp-irregular_past_participle_adjectives', 'social_i_qa', 'anli', 'kilt_zsre', 'cosmos_qa', 'superglue-record', 'squad-with_context', 'emotion', 'blimp-existential_there_quantifiers_1', 'race-middle', 'kilt_wow', 'sciq', 'wino_grande', 'rotten_tomatoes', 'superglue-cb', 'poem_sentiment', 'ropes', 'reddit_tifu-title', 'piqa', 'climate_fever', 'lama-google_re', 'search_qa', 'wiki_auto', 'mc_taco', 'blimp-wh_questions_object_gap', 'hotpot_qa', 'emo', 'kilt_nq', 'kilt_trex', 'quartz-with_knowledge', 'dbpedia_14', 'yahoo_answers_topics', 'app_reviews', 'superglue-copa', 'blimp-anaphor_gender_agreement', 'hate_speech18', 'gigaword', 'multi_news', 'aeslc', 'quail'],
    "dev": ['cos_e', 'kilt_fever', 'eli5-asks', 'trec', 'eli5-eli5', 'art', 'empathetic_dialogues', 'tweet_qa', 'wikisql', 'lama-trex', 'tweet_eval-stance_hillary', 'discovery', 'tweet_eval-emotion', 'liar', 'wiki_bio', 'dream', 'ade_corpus_v2-classification', 'health_fact', 'samsum', 'financial_phrasebank'],
    "test": ['quoref', 'wiki_split', 'ethos-disability', 'yelp_polarity', 'superglue-rte', 'glue-cola', 'ethos-sexual_orientation', 'blimp-sentential_negation_npi_scope', 'ai2_arc', 'amazon_polarity', 'race-high', 'blimp-sentential_negation_npi_licensor_present', 'tweet_eval-irony', 'break-QDMR', 'crawl_domain', 'freebase_qa', 'glue-qnli', 'hatexplain', 'ag_news', 'circa'],
}

\end{lstlisting}

\subsection{Partition 2.1. 45cls}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["superglue-rte", "tweet_eval-sentiment", "discovery", "glue-rte", "superglue-wsc", "scicite", "glue-mrpc", "tweet_eval-stance_hillary", "tweet_eval-offensive", "emotion", "hatexplain", "glue-cola", "sick", "paws", "ethos-sexual_orientation", "glue-qqp", "tweet_eval-emotion", "sms_spam", "health_fact", "glue-mnli", "imdb", "ethos-disability", "glue-wnli", "scitail", "trec-finegrained", "yahoo_answers_topics", "liar", "glue-sst2", "tweet_eval-stance_abortion", "circa", "tweet_eval-stance_climate", "glue-qnli", "tweet_eval-emoji", "ethos-directed_vs_generalized", "ade_corpus_v2-classification", "wiki_auto", "hate_speech_offensive", "superglue-wic", "google_wellformed_query", "tweet_eval-irony", "ethos-gender", "onestop_english", "trec", "rotten_tomatoes", "kilt_fever"],
    "dev": ["tweet_eval-stance_feminist", "ethos-national_origin", "tweet_eval-hate", "ag_news", "amazon_polarity", "hate_speech18", "poem_sentiment", "climate_fever", "medical_questions_pairs", "tweet_eval-stance_atheism"],
    "test": ["superglue-cb", "dbpedia_14", "wiki_qa", "emo", "yelp_polarity", "ethos-religion", "financial_phrasebank", "tab_fact", "anli", "ethos-race"],
}
\end{lstlisting}

\subsection{Partition 2.2. 23cls+22non-cls}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ade_corpus_v2-dosage", "biomrc", "blimp-ellipsis_n_bar_2", "blimp-sentential_negation_npi_scope", "commonsense_qa", "crows_pairs", "duorc", "hellaswag", "kilt_zsre", "lama-google_re", "lama-squad", "math_qa", "numer_sense", "openbookqa", "piqa", "proto_qa", "quartz-no_knowledge", "race-high", "reddit_tifu-tldr", "ropes", "sciq", "wiki_bio", "discovery", "emotion", "ethos-disability", "ethos-sexual_orientation", "glue-cola", "glue-mnli", "glue-mrpc", "glue-qqp", "glue-rte", "glue-wnli", "hatexplain", "health_fact", "imdb", "paws", "scicite", "sick", "sms_spam", "superglue-rte", "superglue-wsc", "tweet_eval-emotion", "tweet_eval-offensive", "tweet_eval-sentiment", "tweet_eval-stance_hillary"],
    "dev": ["tweet_eval-stance_feminist", "ethos-national_origin", "tweet_eval-hate", "ag_news", "amazon_polarity", "hate_speech18", "poem_sentiment", "climate_fever", "medical_questions_pairs", "tweet_eval-stance_atheism"],
    "test": ["superglue-cb", "dbpedia_14", "wiki_qa", "emo", "yelp_polarity", "ethos-religion", "financial_phrasebank", "tab_fact", "anli", "ethos-race"]
}
\end{lstlisting}


\subsection{Partition 2.3. 45non-cls}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ade_corpus_v2-dosage", "art", "biomrc", "blimp-anaphor_number_agreement", "blimp-ellipsis_n_bar_2", "blimp-sentential_negation_npi_licensor_present", "blimp-sentential_negation_npi_scope", "break-QDMR-high-level", "commonsense_qa", "crows_pairs", "dream", "duorc", "eli5-asks", "eli5-eli5", "freebase_qa", "gigaword", "hellaswag", "hotpot_qa", "kilt_ay2", "kilt_hotpotqa", "kilt_trex", "kilt_zsre", "lama-conceptnet", "lama-google_re", "lama-squad", "math_qa", "numer_sense", "openbookqa", "piqa", "proto_qa", "qa_srl", "quarel", "quartz-no_knowledge", "race-high", "reddit_tifu-title", "reddit_tifu-tldr", "ropes", "sciq", "social_i_qa", "spider", "superglue-multirc", "wiki_bio", "wikisql", "xsum", "yelp_review_full"],
    "dev": ["tweet_eval-stance_feminist", "ethos-national_origin", "tweet_eval-hate", "ag_news", "amazon_polarity", "hate_speech18", "poem_sentiment", "climate_fever", "medical_questions_pairs", "tweet_eval-stance_atheism"],
    "test": ["superglue-cb", "dbpedia_14", "wiki_qa", "emo", "yelp_polarity", "ethos-religion", "financial_phrasebank", "tab_fact", "anli", "ethos-race"]
}
\end{lstlisting}

\subsection{Partition 3.1. Held-out-NLI}


\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ade_corpus_v2-classification", "ag_news", "amazon_polarity", "circa", "climate_fever", "dbpedia_14", "discovery", "emo", "emotion", "ethos-directed_vs_generalized", "ethos-disability", "ethos-gender", "ethos-national_origin", "ethos-race", "ethos-religion", "ethos-sexual_orientation", "financial_phrasebank", "glue-cola", "glue-mrpc", "glue-qqp", "glue-sst2", "google_wellformed_query", "hate_speech18", "hate_speech_offensive", "hatexplain", "health_fact", "imdb", "kilt_fever", "liar", "medical_questions_pairs", "onestop_english", "paws", "poem_sentiment", "rotten_tomatoes", "scicite", "sick", "sms_spam", "superglue-wic", "superglue-wsc", "tab_fact", "trec", "trec-finegrained", "tweet_eval-emoji", "tweet_eval-emotion", "tweet_eval-hate", "tweet_eval-irony", "tweet_eval-offensive", "tweet_eval-sentiment", "tweet_eval-stance_abortion", "tweet_eval-stance_atheism", "tweet_eval-stance_climate", "tweet_eval-stance_feminist", "tweet_eval-stance_hillary", "wiki_auto", "wiki_qa", "yahoo_answers_topics", "yelp_polarity"
    ],
    "dev": [],
    "test": ["anli", "glue-mnli", "glue-qnli", "glue-rte", "glue-wnli", "scitail", "sick", "superglue-cb"]
}
\end{lstlisting}


\subsection{Partition 3.2. Held-out-Para}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ade_corpus_v2-classification", "ag_news", "amazon_polarity", "anli", "circa", "climate_fever", "dbpedia_14", "discovery", "emo", "emotion", "ethos-directed_vs_generalized", "ethos-disability", "ethos-gender", "ethos-national_origin", "ethos-race", "ethos-religion", "ethos-sexual_orientation", "financial_phrasebank", "glue-cola", "glue-mnli", "glue-qnli", "glue-rte", "glue-sst2", "glue-wnli", "google_wellformed_query", "hate_speech18", "hate_speech_offensive", "hatexplain", "health_fact", "imdb", "kilt_fever", "liar", "onestop_english", "poem_sentiment", "rotten_tomatoes", "scicite", "scitail", "sick", "sms_spam", "superglue-cb", "superglue-rte", "superglue-wic", "superglue-wsc", "tab_fact", "trec", "trec-finegrained", "tweet_eval-emoji", "tweet_eval-emotion", "tweet_eval-hate", "tweet_eval-irony", "tweet_eval-offensive", "tweet_eval-sentiment", "tweet_eval-stance_abortion", "tweet_eval-stance_atheism", "tweet_eval-stance_climate", "tweet_eval-stance_feminist", "tweet_eval-stance_hillary", "wiki_auto", "wiki_qa", "yahoo_answers_topics", "yelp_polarity"],
    "dev": [],
    "test": ["glue-mrpc", "glue-qqp", "medical_questions_pairs", "paws"]
}

\end{lstlisting}


\subsection{Partition 4.1. Held-out-MRC}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ai2_arc", "aqua_rat", "boolq", "codah", "commonsense_qa", "cosmos_qa", "dream", "eli5-askh", "eli5-asks", "eli5-eli5", "freebase_qa", "hellaswag", "jeopardy", "kilt_hotpotqa", "kilt_nq", "kilt_trex", "kilt_zsre", "lama-conceptnet", "lama-google_re", "lama-squad", "lama-trex", "math_qa", "mc_taco", "numer_sense", "openbookqa", "qasc", "quail", "quarel", "quartz-no_knowledge", "quartz-with_knowledge", "race-high", "race-middle", "sciq", "search_qa", "social_i_qa", "squad-no_context", "superglue-copa", "superglue-multirc", "swag", "web_questions", "wino_grande", "wiqa"
    ],
    "dev": [],
    "test": ["adversarialqa", "biomrc", "duorc", "hotpot_qa", "quoref", "ropes", "squad-with_context", "superglue-record", "tweet_qa"],
}
\end{lstlisting}

\subsection{Partition 4.2. Held-out-MCQA}

\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["adversarialqa", "biomrc", "boolq", "duorc", "eli5-askh", "eli5-asks", "eli5-eli5", "freebase_qa", "hotpot_qa", "jeopardy", "kilt_hotpotqa", "kilt_nq", "kilt_trex", "kilt_zsre", "lama-conceptnet", "lama-google_re", "lama-squad", "lama-trex", "mc_taco", "numer_sense", "quoref", "ropes", "search_qa", "squad-no_context", "squad-with_context", "superglue-multirc", "superglue-record", "tweet_qa", "web_questions"
    ],
    "dev": [],
    "test": ["ai2_arc", "aqua_rat", "codah", "commonsense_qa", "cosmos_qa", "dream", "hellaswag", "math_qa", "openbookqa", "qasc", "quail", "quarel", "quartz-no_knowledge", "quartz-with_knowledge", "race-high", "race-middle", "sciq", "social_i_qa", "superglue-copa", "swag", "wino_grande", "wiqa"]
}
\end{lstlisting}


\subsection{Partition 5. Held-out-GLUE}
To examine whether combining our methods with template-based training \cite{schick2020exploiting,schick2020small,Gao2020MakingPL} results in even better few-shot performance, we add another partition that uses all non-GLUE classification tasks as $\mathcal{T}_{train}$, and all GLUE tasks as $\mathcal{T}_{test}$.
\begin{lstlisting}[language=json,firstnumber=1]
{
    "train": ["ade_corpus_v2-classification", "ag_news", "amazon_polarity", "anli", "circa", "climate_fever", "dbpedia_14", "discovery", "emo", "emotion", "ethos-directed_vs_generalized", "ethos-disability", "ethos-gender", "ethos-national_origin", "ethos-race", "ethos-religion", "ethos-sexual_orientation", "financial_phrasebank", "google_wellformed_query", "hate_speech18", "hate_speech_offensive", "hatexplain", "health_fact", "imdb", "kilt_fever", "liar", "medical_questions_pairs", "onestop_english", "paws", "poem_sentiment", "rotten_tomatoes", "scicite", "scitail", "sick", "sms_spam", "superglue-cb", "superglue-wic", "superglue-wsc", "tab_fact", "trec", "trec-finegrained", "tweet_eval-emoji", "tweet_eval-emotion", "tweet_eval-hate", "tweet_eval-irony", "tweet_eval-offensive", "tweet_eval-sentiment", "tweet_eval-stance_abortion", "tweet_eval-stance_atheism", "tweet_eval-stance_climate", "tweet_eval-stance_feminist", "tweet_eval-stance_hillary", "wiki_auto", "wiki_qa", "yahoo_answers_topics", "yelp_polarity"],
    "dev": [],
    "test": ["glue-cola", "glue-mnli", "glue-mrpc", "glue-qnli", "glue-qqp", "glue-rte", "glue-sst2", "glue-wnli"]
}
\end{lstlisting}

Continued on next page.
